Optimal Branch Exchange for Distribution System Reconfiguration

The feeder reconfiguration problem chooses the on/off status of the switches in a distribution network in order to minimize a certain cost such as power loss. It is a mixed integer nonlinear program and hence hard to solve. A popular heuristic search consists of repeated application of branch exchange, where some loads are transferred from one feeder to another feeder while maintaining the radial structure of the network, until no load transfer can further reduce the cost. Optimizing each branch exchange step is itself a mixed integer nonlinear program. In this paper we propose an efficient algorithm for optimizing a branch exchange step. It uses an AC power flow model and is based on the recently developed convex relaxation of optimal power flow. We provide a bound on the gap between the optimal cost and that of our solution. We prove that our algorithm is optimal when the voltage magnitudes are the same at all buses. We illustrate the effectiveness of our algorithm through the simulation of real- world distribution feeders.

==> tex/2_introduction-v1.tex <==
\section{Introduction}

The topology of a distribution network can be altered by changing the on/off status of section switches on some lines. For example, when a section switch is turned off, the corresponding line is effectively cut off. In normal operation, section switches are configured such that the distribution network is partitioned into several disjoint tree components, called feeders. However, there are many possible configurations and different configurations lead to different aggregate power injection from the substations. 
It is desirable to seek a configuration that minimizes the total amount of power purchased at the substations or minimizes real power loss on the network. 


\slow{Summarize network reconfiguration from \cite{BaranWu}; point out approximation
using "Simplified DistFlow equations" to simplify evaluation of the cost reduction of each
 "open switch".  Here we evaluate this exactly.  Check \cite{feeder1}.}
 
 \slow{Add  pointers to more prior work.}

We define the above problem as an optimal feeder reconfiguration (OFR) problem. In general, the OFR problem seeks to minimize some cost functions by changing the status of the sectioning switches. It is a mixed integer optimization problem with nonlinear power flow constraints, hence difficult to solve. 

Two general approaches are proposed to solve the OFR problem. The first approach uses a iterative greedy like algorithm, \cite{BrananWu, feeder1}. Given a distribution network composed of multiple feeders, they transfer loads from one feeder to another if it gives a smaller cost. The iteration terminates if no loads transfer between two feeders will further decrease the cost. The key challenge is to have an accurate estimate of the change of cost for each loads transfer. The second approach utilizes the mixed integer linear programing solver \cite{MILP}. It takes quite a long time even for small test networks due to its complexity, hence is not applicable in realtime network control. Meanwhile, both approaches rely on linearization of the power flow equations, which are coarse approximations in distribution system. Hence, the accuracy of the algorithms are not guaranteed. 

\subsection*{Summary of Contributions}

The focus of this paper is to propose an efficient algorithm with high degree of accuracy to solve OFR. The main contributions of this paper are threefold:

First, we propose an algorithm to solve the OFR problem that considers the full power flow equations. The algorithm requires solving at most three optimal power flow (OPF) problems, hence is efficient since OPF problem can be solved efficiently by convex program in distribution network under mild conditions. Second, we show our algorithm is accurate in the sense that the gap between the optima of OFR and solution given by our algorithm is negligible under certain conditions. In particular, our algorithm guarantees to find the optima to OFR when the voltage magnitude of each bus is assumed to be the same. Third, we simulated our algorithm in two Southern California Edition (SCE) distribution feeders. The results show that the optima of OFR can always be found.

The rest of the paper is organized as follows. We formulate the optimal feeder reconfiguration problem in section \ref{sec:model} and propose an algorithm to solve it in section \ref{sec:alg}. Theoretical analysis of the performance is given in section  \ref{sec:analysis}. 
The simulation results on SCE distribution circuits are given in section \ref{sec:simulation}. We conclude the paper in section \ref{sec:conclusion}.


